xMLP: Revolutionizing Private Inference with Exclusive Square Activation

Private Inference (PI) enables deep neural networks (DNNs) to work on private data without leaking sensitive information by exploiting cryptographic primitives such as multi-party computation (MPC) and homomorphic encryption (HE). However, the use of non-linear activations such as ReLU in DNNs can lead to impractically high PI latency in existing PI systems, as ReLU requires the use of costly MPC computations, such as Garbled Circuits. Since square activations can be processed by Beaver's triples hundreds of times faster compared to ReLU, they are more friendly to PI tasks, but using them leads to a notable drop in model accuracy. This paper starts by exploring the reason for such an accuracy drop after using square activations, and concludes that this is due to an "information compounding" effect. Leveraging this insight, we propose xMLP, a novel DNN architecture that uses square activations exclusively while maintaining parity in both accuracy and efficiency with ReLU-based DNNs. Our experiments on CIFAR-100 and ImageNet show that xMLP models consistently achieve better performance than ResNet models with fewer activation layers and parameters while maintaining consistent performance with its ReLU-based variants. Remarkably, when compared to state-of-the-art PI Models, xMLP demonstrates superior performance, achieving a 0.58% increase in accuracy with 7x faster PI speed. Moreover, it delivers a significant accuracy improvement of 4.96% while maintaining the same PI latency. When offloading PI to the GPU, xMLP is up to 700x faster than the previous state-of-the-art PI model with comparable accuracy.

==> plots/acc_vs_relu.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    % title={Accuracy vs. ReLU Count},
    xlabel={ReLU Count (K)},
    ylabel={Test Accuracy (\%)},
    xtick={1, 2, 3, 4, 5, 6, 7},
    ymin=59,
    % ytick={0,10,20,30,40,50,60,70,80,90},
    xticklabels={0, 16, 32, 64, 128, 256, 512},
    legend pos=south east,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=solid,
    legend cell align={left},
    legend columns=2, 
    legend style={nodes={scale=0.46, transform shape}}
]

\addplot[
    color=blue,
    mark=*,
    mark options={solid},
    mark size=3pt,
    line width=1pt,
    visualization depends on={value \thisrow{name}\as\modelname},
    nodes near coords={
    \modelname{}
    },
    every node near coord/.append style={anchor=west, font=\small}
    ]
    % coordinates {
    table{
    x y name
    1 75.52 xMLP-M16
    1 76.93 xMLP-M24
    1 78.71 xMLP-T36
    % (6, 2.78)
    };
    \addlegendentry{xMLP(ours)}

\addplot[
    color=brown,
    mark=square,
    mark size=2pt,
    mark options={solid},
    line width=1pt,
    only marks
    % dotted,
    % thick
    ]
    coordinates {
    (4.64, 68.5)
    (6.43, 76.0)
    % (100, 68.5)
    % (344, 76.0)
    };
    \addlegendentry{CryptoNAS}

\addplot[
    color=black,
    mark=triangle,
    mark size=3pt,
    mark options={solid},
    line width=1pt,
    only marks,
    ]
    coordinates {
    (3.64, 63.2)
    (5.5 , 67.2)
    (6.2 , 68.2)
    };
    \addlegendentry{DELPHI}
    
\addplot[
    color=orange,
    mark=+,
    mark options={solid},
    mark size=3pt,
    line width=1pt,
    only marks
    % dotted,
    % thick
    ]
    coordinates {
    (4.75, 67.5)
    % (6, 2.78)
    };
    \addlegendentry{SAFENet}

\addplot[
    color=pink,
    mark=diamond,
    mark options={solid},
    mark size=3pt,
    line width=1pt,
    only marks
    ]
    coordinates {
    (2.678, 66.13) % 25.6
    (3.678, 69.57)
    (4.678, 72.90)
    (5.845, 74.93)
    % (6, 2.78)
    };
    \addlegendentry{Sphynx}

\addplot[
    color=green,
    mark=pentagon,
    mark options={solid},
    mark size=3pt,
    line width=1pt,
    only marks
    ]
    coordinates {
    (1.62,  64.97)
    (2.84,  68.68)
    (3.621, 69.5)
    (5.622, 75.51)
    (5.842, 76.22)
    % (6, 2.78)
    };
    \addlegendentry{DeepReDuce}

\addplot[
    color=red,
    mark=x,
    mark options={solid},
    mark size=3,
    line width=1pt,
    only marks
    ]
    coordinates {
    (1.689, 66.53)
    (1.91,  67.17)
    (2.64,  70.05)
    (3.641, 73.75)
    (4.91,  76.35)
    (5.23,  77.35)
    (5.49,  77.65)
    % (6, 2.78)
    };
    \addlegendentry{SNL}

\end{axis}

\end{tikzpicture}


  \caption{
    xMLP achieves high test accuracy on CIFAR-100 without using any ReLU activation (only square activations), while others selectively replace ReLUs by square activations.
    % xMLP achieves the Pareto frontier on Private Inference Latency vs. test accuracy for CIFAR-100.
    % Comparison of private inference latency under different batch sizes
    % for the proposed xMLP and two SOTA PI implementations (ResNet-18 with garbled circuits and binary secrete sharing for its ReLUs, respectively) on CIFAR-100. More details in Table~\ref{tab:PI_EVAL}.
   % \cref{tab:PI_EVAL}.
    %Comparisons on private inference latency of different batch sizes.} xMLP-S16 and ResNet-18 have 75.52\% and 75.43\% accuracy on CIFAR-100 respectively.
    %While using secret sharing to process all linear layers for all models, we use Beaver Triples to process non-linear layers in xMLP-S16 and garbled circuits/binary secret sharing for non-linear layers in ResNet-18. For a single image, xMLP-S16 takes 0.36 seconds, and ResNet-18 takes 4.17 seconds over garbled circuits and 1.39 seconds over binary secret sharing.
    %Experimental details in \Cref{sec:pi}.
    }
  \label{fig:latency}
  
\vspace{-0.3cm}
\end{figure}

==> plots/breakdown.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=1\linewidth]{assets/breakdown.png}
  
  \caption{
    \textbf{(Sketch) Online Inference Latency Breakdown.} The latency of private inference on a single 32$\times$32 colored image of xMLP-24 and ResNet18. For ResNet18, the private ReLU operation takes 90\% of the time over garbled circuits and 70\% of the time over binary secret sharing. xMLP achieves a much faster the private inference speed by using quadratic activation instead of ReLU to avoid costly garbled circuits or binary secret sharing MPC primitives. Experiments details in \Cref{sec:pi}.}
    
  \label{fig:breakdown}
\end{figure}


==> plots/exp_act_backup.tex <==
% \begin{figure}[t]
\begin{wrapfigure}{r}{0.54\textwidth}
% \vspace{-0.1cm}
    \centering
    \pgfplotsset{xmin=-2, xmax=2, ymin=-0.2, ymax=2, samples=400}

     \begin{subfigure}[b]{0.31\linewidth}
     \centering
            \begin{tikzpicture}[scale=0.35]
            \begin{axis}
              % \addplot[black, ultra thick] (x, x*(x>=0) );
              \addplot[blue, ultra thick] (x, x*(x>0););
            \end{axis}
            \end{tikzpicture}
         \caption{\footnotesize$ReLU(x)$}
         \label{fig:fn_ReLU}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.31\linewidth}
     \centering
            \begin{tikzpicture}[scale=0.35]
            \begin{axis}
              \addplot[black, ultra thick] (x,x*x);
            \end{axis}
            \end{tikzpicture}
         \caption{\footnotesize$x^2$}
         \label{fig:fn_square}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.31\linewidth}
     \centering
            \begin{tikzpicture}[scale=0.35]
            \begin{axis}
              \addplot[black, ultra thick][domain=0:4] (x,x*x*(x>0););
              \addplot[blue, ultra thick][domain=-4:0] (x,x*x*(x>0););
              % \addplot[black, ultra thick] (x*(x>0), x;);
            \end{axis}
            \end{tikzpicture}
         \caption{\footnotesize$ReLU(x)^2$}
         \label{fig:fn_relu_square}
     \end{subfigure}

    % \vspace{-0.1cm}
    \caption{Impacts of various nonlinear activation functions.
    %ReLU drops the negative units, which allows the network to filter redundant information. $y=ReLU(x)^2$ is the combination of square and ReLU function, it has the same ability to drop redundant information like ReLU.
    }
    \label{fig:exp_act_fn}
\end{wrapfigure}
% \end{figure}


==> plots/kernel_visual.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.45\linewidth}
    \centering
    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \includegraphics[height=0.8\linewidth]{assets/square_kernel.png}
    \caption{{\tt square}}
    \label{fig:square-kernel}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\linewidth}
    \centering
    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \includegraphics[height=0.8\linewidth]{assets/relu_kernel.png}
    \caption{ReLU}
    \label{fig:relu-kernel}
  \end{subfigure}
  \caption{
  \textbf{Visualizations of convolutional kernels in xMLP models with different activation functions.} \cref{fig:square-kernel} and \cref{fig:relu-kernel} shows the averaged convolution kernels (from 256 kernels) from the deepest (16$^{th}$) depth-wise convolution layer in {\tt square}-based and ReLU-based xMLP-M16 models. The kernel weights are linearly normalized to reflect how much a kernel aggregates information from nearby units compare to the center unit.}
  \label{fig:visual-kernel}
\end{figure}

==> plots/locality_curve.tex <==
\begin{figure}[t]
% \centering
\resizebox{120pt}{!}{
\begin{tikzpicture}
\begin{axis}[
    title={Avg. Weight vs. Layer Index},
    xlabel={Layer index},
    ylabel={Avg. Weight},
    % xtick={1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15, 16},
    % ytick={0,10,20,30,40,50,60,70},
    % xticklabels={1, 2, 4, 8, 16},
    legend pos=south west,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=solid,
    legend cell align={left},
    legend style={nodes={scale=0.8, transform shape}}
]
\addplot[
    color=blue,
    % mark=square*,
    % mark size=2pt,
    mark options={solid},
    % dotted,
    thick
    ]
    coordinates {
    (1, 0.9393)
    (2, 0.8355)
    (3, 0.9465)
    (4, 0.9266)
    (5, 0.9690)
    (6, 0.9654)
    (7, 0.8567)
    (8, 0.9391)
    (9, 0.8950)
    (10, 0.8314)
    (11, 0.8385)
    (12, 0.7287)
    (13, 0.6695)
    (14, 0.6527)
    (15, 0.7004)
    (16, 0.6992)
    };
    \addlegendentry{Square}
    
\addplot[
    color=red,
    % mark=square*,
    % mark size=2pt,
    mark options={solid},
    % dotted,
    thick
    ]
    coordinates {
    (1, 0.8421)
    (2, 0.8615)
    (3, 0.8882)
    (4, 0.9434)
    (5, 0.8990)
    (6, 0.8610)
    (7, 0.8919)
    (8, 0.8115)
    (9, 0.7472)
    (10, 0.7330)
    (11, 0.7592)
    (12, 0.6068)
    (13, 0.9151)
    (14, 0.4816)
    (15, 0.7385)
    (16, 0.7933)
    };
    \addlegendentry{ReLU}
\end{axis}
\end{tikzpicture}}

  \caption{
    %While using secret sharing to process all linear layers for all models, we use Beaver Triples to process non-linear layers in xMLP-S16 and garbled circuits/binary secret sharing for non-linear layers in ResNet-18. For a single image, xMLP-S16 takes 0.36 seconds, and ResNet-18 takes 4.17 seconds over garbled circuits and 1.39 seconds over binary secret sharing.
    %Experimental details in \Cref{sec:pi}.
    }
  \label{fig:locality}
  
\end{figure}

==> plots/pi_lat.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1\linewidth]{assets/lats.png}
  
%   \caption{
%     \textbf{Online Inference Latency for different batch size} When batch size is 1, xMLP is 2x faster than ResNet18 over BSS. When batch size increase to 32, xMLP becomes 10x faster than ResNet18 under the same setting.
%     }
    
%   \label{fig:latency}
% \end{figure}
\input{plots/plot_lat.tex}

==> plots/plot_lat.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    title={Latency vs. Batch Size},
    xlabel={Batch Size},
    ylabel={Latency (s)},
    xtick={1, 2, 3, 4, 5, 6},
    ytick={0,10,20,30,40,50,60,70},
    xticklabels={1, 2, 4, 8, 16},
    legend pos=north west,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=solid,
    legend cell align={left},
    legend style={nodes={scale=0.8, transform shape}}
]
\addplot[
    color=black,
    mark=square*,
    mark size=2pt,
    mark options={solid},
    dotted,
    thick
    ]
    coordinates {
    (1, 4.17)
    (2, 8.91)
    (3, 15.88)
    (4, 36.71)
    (5, 66.63)
    % (6, 129.67)
    };
    \addlegendentry{ResNet-18 (Garbled Circuits)}

\addplot[
    color=black,
    mark=triangle*,
    mark size=3pt,
    mark options={solid},
    dotted,
    thick
    ]
    coordinates {
    (1, 1.39)
    (2, 2.42)
    (3, 4.65)
    (4, 9.30)
    (5, 18.57)
    % (6, 44.50)
    };
    \addlegendentry{ResNet-18 (Binary Secret Sharing)}
    
\addplot[
    color=blue,
    mark=otimes,
    mark options={solid},
    mark size=3pt,
    dotted,
    thick
    ]
    coordinates {
    (1, 0.36)
    (2, 0.43)
    (3, 0.58)
    (4, 0.86)
    (5, 1.49)
    % (6, 2.78)
    };
    \addlegendentry{xMLP-M16 (Beaver Triples)}
    
\end{axis}

\end{tikzpicture}


  \caption{
    Comparison of private inference latency under different batch sizes
    for the proposed xMLP and two SOTA PI implementations (ResNet-18 with garbled circuits and binary secrete sharing for its ReLUs, respectively) on CIFAR-100. More details in Table~\ref{tab:PI_EVAL}.
   % \cref{tab:PI_EVAL}.
    %Comparisons on private inference latency of different batch sizes.} xMLP-S16 and ResNet-18 have 75.52\% and 75.43\% accuracy on CIFAR-100 respectively.
    %While using secret sharing to process all linear layers for all models, we use Beaver Triples to process non-linear layers in xMLP-S16 and garbled circuits/binary secret sharing for non-linear layers in ResNet-18. For a single image, xMLP-S16 takes 0.36 seconds, and ResNet-18 takes 4.17 seconds over garbled circuits and 1.39 seconds over binary secret sharing.
    %Experimental details in \Cref{sec:pi}.
    }
  \label{fig:latency}
  
\vspace{-0.3cm}
\end{figure}

==> plots/xMLP_activation.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.45\linewidth}
    \centering
    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \includegraphics[height=1\linewidth]{assets/gelu.png}
    \caption{Non-linearity in ResMLP}
    \label{fig:act-gelu}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\linewidth}
    \centering
    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \includegraphics[height=1\linewidth]{assets/qua.png}
    \caption{Non-linearity in xMLP}
    \label{fig:act-qua}
  \end{subfigure}
  \caption{
    Comparison of activation formats in ResMLP and xMLP.
  }
  \label{fig:act}
\end{figure}

==> tables/PI_eval.tex <==
\begin{table*}
\centering
\begin{tabular}{l|l|lccc}
\toprule
 Framework               & Model      & Protocols & \#ReLU (K) & \#Latency (s) & Top-1(\%) \\
\midrule
\multirow{3}{*}{Delphi}  & ResNet18   & GC        & 432        & 10.3          & 75.43      \\
                         & DeepReduce & GC+BT     &            &               &           \\
                         & CNET-C100  & GC+BT     &            &               &           \\
\midrule
\multirow{3}{*}{CrypTen} & ResNet18   & BSS       & 432        & 1.2           &           \\
                         & DeepReDuce & BSS+BT    & 236        &               & 73        \\
                         & xMLP    & BT        & 0          & 0.3           & 75.7     \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/PI_eval_optional.tex <==
\begin{table}[h]
\centering
\scalebox{0.68}{\begin{tabular}{l|cc|l|ccc}
\toprule
\multirow{2}{*}{Model}      & \multirow{2}{*}{\#ReLU (K)} & \multirow{2}{*}{Top-1 (\%)} & \multirow{2}{*}{Protocol} & \multicolumn{3}{c}{Latency (s)} \\ %\cline{5-7}
                            &                             &                            &                           & bs=1     & bs=8     & bs=32     \\ \midrule
    \multirow{2}{*}{ResNet-18\cite{he2016deepres}}   & \multirow{2}{*}{431}        & \multirow{2}{*}{75.43}     & GC                        & 4.17     & 36.71       & 129.67     \\
                            &                             &                            & BSS                       & 1.39      & 9.30 &   44.50      \\ \midrule
                            
\multirow{2}{*}{DeepReduce\cite{jha2021deepreduce}} & \multirow{2}{*}{237}        & \multirow{2}{*}{73.14}     & GC+BT                     & 2.60      & 18.73       & 68.63       \\
                            &                             &                            & BSS+BT                    & 0.85      & 5.19        & 21.16        \\ \midrule
                            
\multirow{2}{*}{DELPHI\cite{mishra2020delphi}} & \multirow{2}{*}{184}        & \multirow{2}{*}{66.70}     & GC+BT                     & 2.34      & 14.90       & 51.90       \\
                            &                             &                            & BSS+BT                   & 0.64      & 2.31 &  8.63      \\ \midrule
% \multirow{2}{*}{Delphi} & \multirow{2}{*}{237}        & \multirow{2}{*}{73.14}     & GC+BT                     & 2.60      & 18.73       & 68.63       \\
                            % &                             &                            & BSS+BT                    & 0.85      & 5.19        & 21.16        \\ \midrule
                            
xMLP-M16          & 0                           & 75.52                      & BT                        & 0.36      & 0.86        & 2.78  \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Comparisons on the online inference latency.} We report the top-1 accuracy on CIFAR-100 and the average online inference latency of five models under different batch size.
DeepReDuce uses a modified ResNet-18 where ReLUs in the first and second block are replaced by quadratic activation. We report its accuracy without knowledge distillation.
DELPHI uses a modified ResNet-32 with 12 ReLU layers replaced by quadratic activation.
``bs'' represents the batch size. ``\#ReLU'' shows the number of individual ReLUs in the network.
}
\label{tab:PI_EVAL}
% \vspace{-0.3cm}
\end{table}

==> tables/ablation_backup.tex <==
% \newcommand{\cyan}{\cellcolor[blue]{0.2}}


\begin{table*}
\centering

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|l|c|l|c}
\toprule
Ablation                         & Model       & Params& Variant                                        & Top-1 (\%) \\ \midrule
\multirow{4}{*}{Baseline models} & xMLP-M16 & 2.2   & 16 layers, embedding dimension 256             & 75.52 \\
                                 & xMLP-M24 & 3.3   & 24 layers, embedding dimension 256             & 76.93 \\
                                 & xMLP-T36 & 10.8  & 36 layers, embedding dimension 384             & 78.71 \\
                                 & xMLP-T48 & 14.4  & 48 layers, embedding dimension 384             & 72.62 \\ \midrule
\multirow{4}{*}{Normalization}   & xMLP-M16 & 2.2   & Per-patch Aff, per-patch BN                    & 75.00 \\
                                 & xMLP-M16 & 2.2   & Per-patch Aff, per-channel BN                  & 74.20 \\
                                 & xMLP-M16 & 2.2   & Per-channel Aff, per-channel BN                & 74.80 \\
                                 & xMLP-M16 & 2.2   & per-channel Aff, per-channel LN                & 75.17 \\ \midrule
\multirow{4}{*}{Activation}      & xMLP-M16 & 2.2   & {\tt square} $\rightarrow$ ReLU                & 76.48 \\
                                 & xMLP-M16 & 2.2   & {\tt square} $\rightarrow$ GELU                & 76.43  \\
                                 & xMLP-M16 & 3.2   & {\tt square} $\rightarrow$ {\tt dotSquare}     & 75.64 \\
                               % & xMLP-M24 &       & \tt square $\rightarrow$ \tt dotSquare         & 76.58 \\
                               % & xMLP-B36 & 16.1  & \tt square $\rightarrow$ \tt dotSquare         & 77.95 \\
                                 & xMLP-T48 & 21.5  & {\tt square} $\rightarrow$ {\tt dotSquare}     & 76.49 \\ \midrule
\multirow{3}{*}{Patch mixer} & xMLP-M16     & 2.2   & 3$\times$3 dconv $\rightarrow$ none            & 58.82 \\
                                 & xMLP-M16 & 2.2   & 3$\times$3 dconv $\rightarrow$ linear          & 73.13 \\
                               % & xMLP-M24 & 3.3   & 3$\times$3 dconv $\rightarrow$ linear          & 75.57 \\
                               % & xMLP-T36 & 14.4  & 3$\times$3 dconv $\rightarrow$ linear          & 77.17 \\
                                 & xMLP-M16 & 11.6  & 3$\times$3 dconv $\rightarrow$ 3$\times$3 conv & 77.28 \\  \midrule
                               % & xMLP-B48 &       & dconvolution $\rightarrow$ linear              & 76.49 \\
\multirow{1}{*}{Channel Mixer}  & xMLP-M16  & 19.0  & linear $\rightarrow$ 3$\times$3 conv           & 73.63  \\ \midrule
\multirow{3}{*}{Patch Mixer \& Activation}  & xMLP-M16 &  2.2     & 3$\times$3 dconv $\rightarrow$ linear, {\tt square} $\rightarrow$ ReLU & 73.67 \\
                                 & xMLP-M16 &  2.2  & 3$\times$3 dconv $\rightarrow$ linear, {\tt square} $\rightarrow$ GELU            &  74.49 \\
                                 & xMLP-M16 &  3.3  & 3$\times$3 dconv $\rightarrow$ linear, {\tt square} $\rightarrow$ {\tt dotSquare} &   74.46    \\
\bottomrule
\end{tabular}

\label{tab:ablation}
\caption{\textbf{Ablation on CIFAR-100.} 
We report top-1 accuracy on the test set of CIFAR-100.
"dconv" stands for the depth-wise convolution, while "conv" stands for the standard convolution.
}
\end{table*}

==> tables/cifar100.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{l|ccc}
\toprule
Models                                  & Activation          & Params (M)  & Top-1 (\%) \\ \midrule
ResNet-18            & ReLU                & 11.4        & 75.43      \\
ResNet-34            & ReLU                & 21.3        & 76.73      \\
ResNet-50            & ReLU                & 23.7        & 77.44      \\
ResNet-164            & ReLU                & 1.7        & 75.67      \\
\midrule
% Mixer-S/4\cite{tolstikhin2021mlpmixerw}           & GELU          & 17.2        & 69.76      \\
% Mixer-N/4$^\dagger$\cite{tolstikhin2021mlpmixer} & GELU          &             & 70.23      \\
ResMLP-S12               & GELU          & 14.3        & 74.02      \\
ResMLP-S24              & GELU          & 28.5        & 75.56      \\
ResMLP-M16     & GELU          & 2.2         & 68.19      \\
ResMLP-M24     & GELU          & 3.3         & 67.67      \\
% ResMLP-M36$^\dagger$ \cite{touvron2022resmlp}    & GELU          &             &            \\
xMLP-M16 (Ours)                               & Square   & 2.2         & 75.52      \\
xMLP-M24 (Ours)                               & Square   & 3.3         & 76.93      \\
xMLP-T36 (Ours)                               & Square   & 10.8        & 78.71      \\ \bottomrule
\end{tabular}}
\caption{\textbf{Performance Comparison on CIFAR-100.} We report Top-1 accuracy on the test set of CIFAR-100 with parameter sizes and activation function used. All Models are trained on CIFAR-100 from scratch. ResMLP models follow the architecture in \cite{touvron2022resmlp} and configurations in \Cref{tab:xMLP-config}. ResNet-18/34/50 follow the architectures in \cite{he2016deepres} while the first convolution layer uses the 3x3 convolution kernel, ResNet-164 is a light-weight model from \cite{he2016identity}.
%All the models use 32$\times$32 images as input. Mixer, ResMLP and xMLP models all uses 8$\times$8 patches of size 4$\times$4. $\dagger$ models use xMLP's configurations. 
% Mixer-S/4 uses the same configuration as Mixer-S/32 as in~\cite{tolstikhin2021mlpmixer} except that the patch size is set to 4.
%The number of parameters and FLOPS are calculated based on an input resolution of 32×32. The FLOPS are counted by OpCounter\cite{OpCount} library.
}

\label{tab:cifar100}
\end{table}


% \begin{table}[ht]
% \centering
% \begin{tabular}{c|l|ccc}
% \toprule
% General Arch                 & Models                                  & Activation          & Params (M)  & Top-1 (\%) \\ \midrule
% \multirow{2}{*}{Convolution} & ResNet18\cite{he2016deepres}            & ReLU                & 11.4        & 75.43      \\
%                              & ResNet34\cite{he2016deepres}            & ReLU                & 21.3        & 76.73      \\
%                              % & ResNet18-deepreduce\cite{jha2021deepreduce}            & ReLU+\tt{square}  &  98  & 1.98 &   11.2     &     68.4   \\ 
%                              % & ResNet18-deepreduce\cite{jha2021deepreduce}            & ReLU+\tt{square}  &  197  & 3.98 &   11.2       &     72.77   \\ 
%                              % & ResNet18-deepreduce\cite{jha2021deepreduce}            & ReLU+\tt{square}  &  229   & 4.63 &   11.2    &     73.14   \\ 
%                              % & CNET-C100\cite{cryptonas}             & ReLU+\tt{square} &  86  & 1.74  &   1.3  &     68.13   \\ 
%                              % & CNET-C100\cite{cryptonas}             & ReLU+\tt{square} &  344  & 6.96 &    15  &     75.64   \\ 
% \midrule
% % \multirow{2}{*}{Vision Transformer} & ViT\cite{he2016deepres}        & GELU                &             &            \\
% %                              & ViT\cite{he2016deepres}               & GELU                &             &            \\ \midrule
% \multirow{6}{*}{MLP}         & Mixer-S/16\cite{tolstikhin2021mlpmixer} & GELU                &             & 70.23      \\
%                              & Mixer-S/16$^\dagger $ \cite{tolstikhin2021mlpmixer}       & \tt{quadratic}      &             & 70.68      \\
%                              & ResMLP-S24\cite{touvron2022resmlp}      & GELU                & 3.3         & 75.11      \\
%                              & ResMLP-B36\cite{touvron2022resmlp}      & GELU                &             & 76.76      \\
%                              & xMLP-S16 (Ours)                      & \tt{square}         & 2.2         & 75.52      \\
%                              & xMLP-S24 (Ours)                      & \tt{square}         & 3.3         & 76.93      \\
%                              & xMLP-L36 (Ours)                      & \tt{square}         & 10.8        & 78.71      \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Performance Comparison on CIFAR-100.} All Models are trained on CIFAR-100 from scratch. Mixer-S/16$^\dagger$ replaces GELU and LayerNorm by {\tt quadratic} activation and batch normalization respectively.
% %The number of parameters and FLOPS are calculated based on an input resolution of 32×32. The FLOPS are counted by OpCounter\cite{OpCount} library.
% }

% \label{tab:cifar100}
% \end{table}

==> tables/imnet.tex <==
% \begin{table}[t]
\begin{wraptable}{R}{0.5\textwidth}

\centering
\resizebox{0.8\linewidth}{!}{

\begin{tabular}{@{}l|ccc@{}}
\toprule
Dataset                        & Models     & Activation & Top-1 (\%) \\ \midrule
\multirow{3}{*}{Tiny-ImageNet} & xMLP-M16  & Square     & 63.84\%    \\
                               & xMLP-M16  & ReLU       & 64.59\%    \\
                               & ResNet-18 & Square     & 63.68\%    \\ \midrule
\multirow{2}{*}{ImageNet}      & xMLP(20M) & Square     & 72.83\%    \\
                               & xMLP(20M) & ReLU       & 70.20\%    \\ \bottomrule
\end{tabular}
}
\caption{
Test Accuracy on Tiny ImageNet and ImageNet.
}
\label{tab:imagenet}
% \end{table}
\end{wraptable}

==> tables/polynomial.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
    \toprule
  Notation  & Activation Format    & Degree \\
    \midrule
   \tt square  & $(WX)\circ(WX)$ \cite{gilad2016cryptonets}          & 2  \\
   \tt dotSquare & $(W_1X)\circ(W_2X)$ \cite{bu2021quadratic}& 2  \\
    \bottomrule
    \end{tabular}
\caption{\textbf{Two representative quadratic activation functions.} $X$ is the layer input; $W, W_1, W_2$ are the learnable weight matrix of the pre-activation linear layer; and $\circ$ denotes the element-wise multiplication. 
}
\label{tab:poly}
% \vspace{-0.3cm}
\end{table}

==> tables/spec.tex <==
% \begin{table}[h!]
\begin{wraptable}{R}{0.5\textwidth}
\centering
% \vspace{-0.3cm}
\begin{tabular}{@{}lccc@{}}
  \toprule
  % Specification       & 
  Configurations             & M    & T   & S    \\
  \midrule
  Image size                 & 32   & 32  & 32   \\
  Patch size                 & 4    & 4   & 4    \\
  Embedding dimension        & 256  & 384 & 512  \\
  Channel-mixing dimension   & 256  & 384 & 2048 \\
  Patch-mixing dimension     & 64   & 64  & 64   \\
  % Parameters (M)                  & 4.9       & 3.3               \\
  \bottomrule
\end{tabular}
% \vspace{-0.1cm}
\caption{
  Model configurations.% The ``M'', ``T'' and ``S'' denote ``mini'' and ``tiny'' configurations, respectively, for xMLP, while ``S'' denotes the small configuration for ResMLP~\cite{touvron2022resmlp} by adjusting their image and patch sizes according to CIFAR-100.
  % xMLP do not expand the dimension of the embeddings in the channel-mixer, as it increases the computation for activation layers which is more expensive than linear operations in PI.
 }
 \label{tab:xMLP-config}
% \label{tab:spec}
% \vspace{-0.3cm}
\end{wraptable}

